Jam-X: Wireless Agreement under Interference

Wireless low-power transceivers used in sensor networks such as IEEE 802.15.4 typically operate in unlicensed frequency bands that are subject to external interference from devices transmitting at much higher power. Communication protocols should therefore be designed to be robust against such interference. A critical building block of many protocols at all layers is agreement on a piece of information among a set of nodes. At the MAC layer, nodes may need to agree on a new time slot or frequency channel; at the application layer nodes may need to agree on handing over a leader role from one node to another. Message loss caused by interference may break agreement in two different ways: none of the nodes use the new information (time slot, channel, leader) and stick with the previous assignment, or - even worse - some nodes use the new information and some do not. This may lead to reduced performance or failures. In this paper we investigate the problem of agreement under interference and point out the limitations of the traditional message-based n-way handshake approach. We propose novel protocols that use jamming instead of message transmissions and show that they outperform the n-way handshake in terms of agreement probability, energy consumption, and time-to-completion both in the unicast case (two neighboring nodes agree) as well as in the broadcast case (any number of neighboring nodes agree).

==> Makefile <==
# PLEASE TYPE  $ make IN THE COMMAND LINE TO GENERATE THE PDF (NO  $ make paper.pdf) #
default: paper.pdf
FIGURES= figures/p_positive_agreement_3d.eps figures/p_negative_agreement_3d.eps figures/p_disagreement_3d.eps \
		 figures/p_positive_agreement.eps figures/p_disagreement.eps \
		 figures/scanner_heavy_wifi.eps figures/scanner_heavy_wifi_2.eps figures/scanner_no_interf.eps \
	     figures/scanner_microwave.eps figures/scanner_jammer.eps figures/scanner_zigbee.eps figures/scanner_bluetooth.eps \
		 figures/scanner_wifi_ontop.eps \
		 figures/ACK2_bluetooth.eps figures/ACK2_microwave.eps figures/ACK2_wifi.eps \
		 figures/JAM2_bluetooth.eps figures/JAM2_microwave.eps figures/JAM2_wifi.eps \
		 figures/ACK_handshake_bluetooth.eps figures/ACK_handshake_microwave.eps figures/ACK_handshake_wifi.eps \
		 figures/ACK2_power_bluetooth.eps figures/ACK2_power_microwave.eps figures/ACK2_power_wifi.eps \
		 figures/JAM2_power_bluetooth.eps figures/JAM2_power_microwave.eps figures/JAM2_power_wifi.eps \
		 figures/JAM2_ACK2_power_bluetooth.eps figures/JAM2_ACK2_power_microwave.eps figures/JAM2_ACK2_power_wifi.eps \
		 figures/ACK2_disagreements.eps figures/JAM2_disagreements.eps \
		 figures/tx_delay.eps figures/tx_delay_2.eps figures/tx_delay_3.eps \
		 figures/JAM3_3d_bluetooth_disagreements.eps figures/JAM3_3d_bluetooth_positive_agreements.eps figures/JAM3_3d_bluetooth_negative_agreements.eps \
		 figures/JAM3_3d_microwave_disagreements.eps figures/JAM3_3d_microwave_positive_agreements.eps figures/JAM3_3d_microwave_negative_agreements.eps \
		 figures/JAM3_3d_wifi_disagreements.eps figures/JAM3_3d_wifi_positive_agreements.eps figures/JAM3_3d_wifi_negative_agreements.eps \
		 figures/JAM3_2d_bluetooth_disagreements.eps figures/JAM3_2d_bluetooth_positive_agreements.eps figures/JAM3_2d_bluetooth_negative_agreements.eps \
		 figures/JAM3_2d_microwave_disagreements.eps figures/JAM3_2d_microwave_positive_agreements.eps figures/JAM3_2d_microwave_negative_agreements.eps \
		 figures/JAM3_2d_wifi_disagreements.eps figures/JAM3_2d_wifi_positive_agreements.eps figures/JAM3_2d_wifi_negative_agreements.eps \
		 figures/JAM2_time_1.eps figures/JAM2_time_2.eps figures/JAM2_time_3.eps \
		 figures/ACK3_RSSI.eps figures/JAM3_2d_bluetooth_threshold_rssi.eps figures/JAM3_2d_microwave_threshold_rssi.eps figures/JAM3_2d_wifi_threshold_rssi.eps\
		 figures/ACK3.eps figures/JAM3.eps figures/ACK3_JAM3.eps \
		 figures/ACKB_2_bluetooth.eps figures/ACKB_2_microwave.eps figures/ACKB_2_wifi.eps \
		 figures/ACKB.eps figures/JAMB.eps figures/JAMB_2.eps figures/ACKB_JAMB.eps figures/ACKB_JAMB_2.eps \
		 figures/CCA_ACK_handshake_bluetooth.eps figures/CCA_ACK_handshake_microwave.eps figures/CCA_ACK_handshake_wifi.eps \
		 figures/CCA_ACK2_bluetooth.eps figures/CCA_ACK2_microwave.eps figures/CCA_ACK2_wifi.eps \
		 figures/CCA_JAM2_bluetooth.eps figures/CCA_JAM2_microwave.eps figures/CCA_JAM2_wifi.eps \
		 figures/CCA_ACK3.eps figures/CCA_JAM3.eps figures/CCA_ACK3_JAM3.eps figures/CCA_JAM3_RSSI.eps \
		 figures/CCA_ACKB_JAMB.eps \
		 figures/CCA_ACK3_JAM3_NACK.eps figures/CCA_JAM3_NACK_RSSI.eps \
		 figures/JAM2_ACK2_disagreements.eps figures/JAM2_ACK2_disagreements_multiplot.eps figures/JAM2_ACK2_disagreements_bluetooth.eps figures/JAM2_ACK2_disagreements_microwave.eps figures/JAM2_ACK2_disagreements_wifi.eps \
		 figures/JAM2_ACK2_disagreements_2.eps figures/JAM2_ACK2_disagreements_2_multiplot.eps \

#PAPER=a4
PAPER=letter

.PHONY: figures
figures: $(FIGURES)
	@echo "All figures ok"

%.eps: %.fig
	fig2dev -L eps $< $@

%.eps: %.gnuplot %.dat
	gnuplot < $<

%.bibtex: %.tex
	latex ${basename $@} && bibtex ${basename $@}

%.gv: $(FIGURES) %.bibtex %.ps
	gv $@.ps

%.dvi: %.tex figures
	latex ${basename $@} && latex ${basename $@}

%.ps: %.dvi figures
	#dvips -P cmz -t $@ -f $< > $@
	dvips -t ${PAPER} -Ppdf -Pdownload35 -G0 -j0 -sPAPERSIZE=${PAPER} $<

%.pdf: %.ps
	#ps2pdf $< $@
	#bibtex ${basename $@}.aux
	ps2pdf -sPAPERSIZE=${PAPER} -dPDFSETTINGS=/printer -dMaxSubsetPct=100 -dCompatibilityLevel=1.7 -dSubsetFonts=true -dEmbedAllFonts=true $< $@

#%.pdf: %.dvi
#	dvipdf $<

clean:
	-rm $(FIGURES) *.ps *.pdf *.dvi *.aux *.bbl *.blg *.dvi *.log *.out


==> model.tex <==
\section{Model}

%\subsection{Problem Definition}
%
%When two nodes, $\mathcal{A}$ and $\mathcal{B}$, need to agree on a common value, a sequence of $n$ messages is exchanged in an alternated manner. The node that starts the exchange is referred to as the \emph{sender} and the other node as the \emph{receiver}. A node can not send message $i$ until it receives message $i\!-\!1$. If a message is lost, the exchange stops (there are no retransmissions of the same message). Each node uses a simple rule to determine the success of the exchange: if all expected messages are received, the exchange is deemed successful. This scenario leads to three possible outcomes:
%
%\begin{definition}[Agreement] All messages are received. In this case, both nodes receive all the expected messages, and hence, both deem the exchange as successful.
%\label{def.agree}
%\end{definition}
%
%\begin{definition}[Disagreement] The last message is lost. In this case, the receiver gets all the expected messages and deems the exchange successful, but the sender misses the last one and deems the exchange as unsuccessful.
%\label{def.disagree}
%\end{definition}
%
%\begin{definition}[Failed Exchange] A message prior to the last one is lost. In this case, neither node receives all the expected messages, and hence, both deem the exchange as unsuccessful.
%\label{def.fail}
%\end{definition}
%
%Notice that a \emph{Disagreement} is a potentially pernicious outcome, but a \emph{Failed Exchange} is not. For example, two nodes are better of staying in the same lossy wireless channel, than having only one of them move to a different channel.
%
%The frequency of the outcomes described above depend on the link quality. Letting $p$ represent the probability that a message is successfully received and $n$ represent the number of messages, we obtain:
%\begin{eqnarray}
%\text{Prob} ( Agreement ) &=& p^n \nonumber \\
%\text{Prob} ( Disagreement ) &=& p^{n-1} (1-p) \nonumber \\
%\text{Prob} ( Failed~Exchange ) &=& 1 - p^{n-1} \nonumber
%\label{eq.prob}
%\end{eqnarray}
%
%Given that our goal is to increase the frequency of agreements, let us compare two ratios: \emph{Agreement} versus \emph{Disagreement} $(\frac{p}{1-p})$ and \emph{Agreement} versus \emph{Failed Exchange} $(\frac{p^n}{1-p^{n-1}})$. The first ratio indicates that the number of messages $n$ does not play a role, more agreements are simply obtained by increasing the quality of communication. The second ratio indicates that increasing the communication quality or decreasing the number of messages leads to more greements. Hence, we should aim for a mechanism that uses as few messages as possible and high quality channels. In our work, we increase the communication quality by using jamming signals instead of packet transmissions, and we evaluate the proposed jamming methods on 2-way and 3-way handshakes -- in order to use as few messages as possible. 
% 
%\fmmz{Here we describe results and figures}
%
%\subsection{Main Idea}
%
%Our work is motivated by the following observation: in several scenarios, only the first message conveys descriptive information (for example, ``switch to channel $x$''), the remaining messages convey only binary information (``got it''). In terms of radio communication, this observation indicates that only the first message requires a packet transmission, and the other messages require a simple binary signal. The main idea of our work is to use jamming as \emph{the} simple binary signal.
%
%After the transmission of the first packet, the subsequent acknowledgments can be sent in the form of jamming signals. Under the presence of interference, detecting jamming signals have a significantly higher probability than successfully decoding and ACK packet.  
%
%\subsection{Jam-2-way}
%
%If the first message is received successfully, the \emph{receiver} sends a jamming signal for a period $t_j$. Meanwhile, the \emph{sender} carries a CCA check for two different periods, $t_x$ and $t_y$. The relationship between $t_j$, $t_x$ and $t_y$ is depicted in Figure X. The period $t_x$ should be less than $t_j$ and synchronized in such a way that it is active only when the jamming signal is on the air. The period $t_y$ is used to verify that the receiver stops transmitting the jamming signal. The periods $t_x$ and $t_y$ can be sampled continuously, but differentiating the periods leads to a simpler implementation on the motes.
%
%Denoting $r_n$ as the maximum noise floor measured without interference, and $\{x_1, x_2, \ldots\}$ as the sequence of noise floor values measured during $t_x$, we define the binary sequence $\{X_1, X_2, \ldots\}$ as follows: if $x_i \le r_n$, then $X_i=0$, else $X_i=1$. The binary sequence $\{Y_1, Y_2, \ldots\}$ is similarly defined for the period $t_y$. Now, we define two parameters:
%\begin{eqnarray}
%S_x = \sum_{i=1} X_i \nonumber\\
%S_y = \sum_{i=1} Y_i \nonumber
%\end{eqnarray}
%If $S_x\!=\!0$ and $S_y\!>\!0$, the sender assumes that the jamming sequence was transmitted by the receiver, and hence, an agreement is reached.
%
%\subsection{Jam-3-way}
%
%If the first message is received successfully, the \emph{receiver} sends an acknowledgment packet. If the \emph{sender} receives the ACK it deems the exchange as successful and does nothing else, otherwise, the sender starts a jamming signal for a period $t_j$. Meanwhile, the receiver starts a CCA check for a period $t_w$. If the receiver detects a jamming signal from the sender it deems the exchange as unsuccessful, else, the exchange is considered successful.
%
%The advantage of this approach is that the receiver knows the signal strength of the first packet (RSSI). Considering that the jamming signal has a similar strength to the RSSI of the first packet, this method is better suited to distinguish if the jamming comes from the sender or not. Recall that in Jam-2-way, the sender simply looks for \emph{any} jamming.
%
%Denoting $r_s$ as the RSSI of the first packet (measured at the receiver), and $W=\{w_1, w_2, \ldots\}$ as the sequence of noise floor values measured during $t_w$, we define the binary sequence $\{W_1, W_2, \ldots\}$ as follows: if $|w_i - r_s| \le \Delta r$, then $W_i=1$, else $W_i=0$, where $\Delta r$ checks if the strength of the jamming signal is similar to $r_s$. We define the following parameter:
%\begin{eqnarray}
%S_w = \sum_{i=1} W_i \nonumber
%\end{eqnarray}
%Letting $|W|$ be the number of samples in $W$, $min_W$=$\min\{W\}$ and $max_W$=$\max\{W\}$, the receiver deems the event as unsuccessful iff:
%\begin{eqnarray}
%\frac{S_w}{|W|} > \frac{2\Delta r}{(max_W - min_W)} \nonumber 
%\end{eqnarray}
%The expression above indicates that the jamming obtained around $r_s$  is not simply the result of a uniform random signal, but there is indeed a source (sender) that is pursposedly sending this signal.


Given an interference source $\mathcal{I}$ (WiFi, Bluetooth, Oven), let $X_{\mathcal{I}}$ and $Y_{\mathcal{I}}$ be random variables representing the length of their idle and interfering periods. For example, \fmmz{Here we need two figures two depict the distributions of these random variables.}.

\subsection{Parameter Calibration for Jam-2}

In order for Jam-2 to be successful (positive agreement), two conditions must be
satisfied: (i) the packet from node $\mathcal{A}$ to node $\mathcal{B}$ must be
successfully decoded and (ii) node $\mathcal{A}$ must unequivocally determine
that the jamming signal came from node $\mathcal{B}$ \fmcb{Warning! We are not
able to unequivocally determine that it was node B and not node C!}. The success
of condition (i) depends on the interplay of $X_{\mathcal{I}}$ (length of idle
periods) and the transmission delay of the packet $t_pkt$, and the success of
condition (ii) depends on the interplay of $Y_{\mathcal{I}}$ (length of
interfering periods) and the length of the jamming signal $t_{jam}$. We now
analyze these two conditions in greater detail.


\textbf{Successful reception of packet.} Given the current RF (radio frequency)
technology utilized in sensor nodes, a packet can only be successfully decoded
if it is transmitted during an idle period \fmcb{what about FEC techniques?}.
For periodic sources, such as microwave ovens, the idle period is rather
constant and we denote it by $t_{off}$. For more random sources, different
models have been developed to capture the probability density function\fmmz{Here
we need references from Jamlab}. In our study, however, we use a simple
exponential distribution ($F(X)=1-\exp^{-\lambda x}$) to illustrate the
importance of calibrating the parameters of Jam-2. Figure\fmmz{Here we need a
figure with curve fits} shows an MMSE approximation of a X source to an
exponential distribution.


Assuming that node $\mathcal{B}$ is within range of $\mathcal{A}$, the probability of successfully delivering the packet is given by:

\begin{equation}
\text{Prob(packet success | periodic source)} = \frac{\max\{t_{off}-t_{pkt} , 0\}}{t_{off}}
\label{eq.pkt_success_per}
\end{equation} 

\begin{equation}
\text{Prob(packet success | exponential source)} = \exp^{-\lambda t_{pkt}}
\label{eq.pkt_success_exp}
\end{equation} 

The equations above simply state the probability that the transmission delay fits within the idle period. For the exponentially sources, $\lambda = \frac{1}{\text{average idle time}}$. 

The equations above provide two important trends. First, it allows us to quantify the success of Jam-2. For instance, for the parameters evaluated in Section X\fmmz{Here we need the parameters of the evaluation to see if there is indeed a connection}. Second, it permits us to compare the performance of Jam-2 with respect to Ack-2. For example, for ACK-2 instead of utilizing only $t_{pkt}$ we would need $t_{pkt} + t_{ack}$, that is, we require an empty period sufficiently large to contain the packet and the acknowledgment. For the parameters used in the evaluation this would lead to \fmmz{Here we need the parameters of teh evaluation to give data}

\textbf{Successful identification of jamming signal.} In Jam-2, a sending node samples the channel to listen for a jamming signal for a period $t_{jam}$. However, this signal can be confused with any other interference. In order to guarantee that the signal unequivocally belongs to the Jam-2 exchange $t_{jam}$ should be longer than the maximum interference period. Formally, a sufficient condition for this to happen is that $t_{jam} > \max\{Y_{\mathcal{I}}\}$. Contrary to the idle periods which have a large deviation, the interference periods are bounded by the minimum and maximum frame size of the interference source. Hence, it is simpler to identify $t_{jam}$. For the sources evaluated in Section X, we find that periods of X,Y,Z, are sufficient for sources X,Y,Z, respectively. 

It is important to notice that in Jam-2, having $t_{jam} < \max\{Y_{\mathcal{I}}\}$ can lead to false positive agreements. In practice, a false positive is the same as as having a disagreement, and hence, it is a highly undesirable outcome. Jam-2 overcomes the limitations of its simple mechanism by extending the length of the sampling period $t_{jam}$, which consumes more energy and leads to longer delays. 

Overall, if $t_{jam} > \max\{Y_{\mathcal{I}}\}$, the success probability (positive agreement) of Jam-2 is largely determined by equations~\ref{eq.pkt_success_per} and~\ref{eq.pkt_success_exp}.

\subsection{Parameter Calibration for Jam-3.} The analysis of Jam-3 is similar to Jam-2 but it has some differences that are important to highlight. Jam-3 must satisfy two conditions: (i) the idle time should be longer than in Jam-2 to accommodate a packet and an acknowledgment and (ii) unequivocally identifying the jamming signal (or lack of) does not require a sampling window longer than $\max \{Y_{\mathcal{I}} \}$.

Replacing $t_{pkt}$ with $t_{pkt} + t_{ack}$ in equations~\ref{eq.pkt_success_per} and~\ref{eq.pkt_success_exp} provides the packet success probability for Jam-3. It is important to notice that Jam-3 and Ack-2 have the same probability, but Jam-3 provides a higher robustness by utilizing a 3-way handshake.

Contrary to Jam-2, Jam-3 can utilize sampling windows shorter than $\max\{Y_{\mathcal{I}}\}$ because it can discern (to some extent) the jamming signal coming from the receiver. The chances of false positives (disagreements) appear if two conditions are met (i)  $t_{jam} < \max\{Y_{\mathcal{I}}\}$ and (ii) the RSSI of nearby sources are similar to the RSSI of the receiver. In practice, the changes of false positives increases with node/interferer density and high traffic rates. Because more node have a higher chance a similar signal at the time where $t_{jam}$ is being performed. Similarly to Jam-2, false positives can be eliminated if $t_{jam} > \max\{Y_{\mathcal{I}}\}$
